Zero-shot Learning with Class Description Regularization

The purpose of generative Zero-shot learning (ZSL) is to learning from seen classes, transfer the learned knowledge, and create samples of unseen classes from the description of these unseen categories. To achieve better ZSL accuracies, models need to better understand the descriptions of unseen classes. We introduce a novel form of regularization that encourages generative ZSL models to pay more attention to the description of each category. Our empirical results demonstrate improvements over the performance of multiple state-of-the-art models on the task of generalized zero-shot recognition and classification when trained on textual description-based datasets like CUB and NABirds and attribute-based datasets like AWA2, aPY and SUN.

==> figs/tab_attribute_results.tex <==
\begin{table*}[t]
  \centering
%   \begin{tabular}{ >{\columncolor[HTML]{b8e6bf}} c c c c c c c }
  \begin{tabular}{ c c c c c c c }
 \hline
%  \rowcolor[HTML]{b8e6bf}
 Metric & \multicolumn{3}{c}{Top-1 Accuracy (\%)} & \multicolumn{3}{c}{Seen-Unseen H (\%)} \\
%  \rowcolor[HTML]{b8e6bf}
 Dataset & AWA2 & SUN & APY & AWA2 & SUN & APY\\
 \hline
 GAZSL \cite{Yizhe_ZSL_2018} & \iffalse (–lr 0.00005 –zdim 100 –isval)\fi 56.33 & \iffalse –lr 0.0001 –zdim 100 –isval) \fi 60.76 & \iffalse (–lr 0.0001 –zdim 100 –isval) \fi 27.18 & 28.36 & 25.59 & 14.77 \\
 CIZSL \cite{Mohamed_Creative_2019} & \iffalse –lr 0.00005 –zdim 100 –isval) \fi 56.13 & \iffalse (–lr 0.0001 –zdim 10 –isval \fi 61.52& \iffalse (–lr 0.0001 –zdim 100 –isval) \fi 30.98 & 26.66 & 26.27 & 16.31 \\
 \hline
 DGRZSL & \iffalse –lr 0.0001 –zdim 100 –isval) \fi \textbf{57.79} & \iffalse  (–lr 0.0001 –zdim 10 –isval) \fi \textbf{61.94} & \iffalse –lr 0.00005 –zdim 100 –isval) \fi \textbf{38.59} & \textbf{33.50} & \textbf{26.70} & \textbf{18.09} \\
 \hline
\end{tabular}
  \caption{Zero-Shot classification results on AWA2, SUN and APY datasets. Our model outperforms both baseline models in all cases with an average top-1 accuracy increase of 9.4 \% and seen-unseen H increase of 17.26\% over CIZSL}
  \label{tab:attribute_results}
\end{table*}


==> figs/tab_attribute_results_original_method.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}{ c c c c c c c }
 \hline
 Metric & \multicolumn{3}{c}{Top-1 Accuracy (\%)} & \multicolumn{3}{c}{Seen-Unseen H (\%)} \\
 Dataset & AWA2 & SUN & APY & AWA2 & SUN & APY\\
 \hline
 GAZSL \cite{Yizhe_ZSL_2018} & \iffalse (–lr 0.00005 –zdim 10)\fi 66.44 & \iffalse GAZSL (–lr 0.0001 –zdim 10) \fi 61.31 & \iffalse –lr 0.0001 –zdim 100) \fi \textbf{45.38} & 34.49 & 27.71 & 23.80 \\
 CIZSL \cite{Mohamed_Creative_2019} & \iffalse (–lr 0.0001 –zdim 10)\fi 68.81 & \iffalse –lr 0.0001 –zdim 10) \fi 61.25 & \iffalse –lr 0.0001 –zdim 100 \fi 39.50 & 34.72 & 27.12 & 23.85 \\
 \hline
 DGRZSL & \iffalse (–lr 0.0001 –zdim 10) \fi \textbf{72.02} & \iffalse (–lr 0.0001 –zdim 10)  \fi \textbf{61.73}& \iffalse (–lr 0.0001 –zdim 100) \fi 37.39& \textbf{47.53} & \textbf{28.02} & \textbf{28.4} \\
 \hline
\end{tabular}
  \caption{\added{Zero-Shot classification results on AWA2, SUN and APY datasets using the original evaluation method}}
  \label{tab:attribute_results_original_method}
\end{table*}


==> figs/tab_textual_results.tex <==
\begin{table*}[t]
  \centering
%   \begin{tabular}{ >{\columncolor[HTML]{f5e6ab}} c c c c c c c c c }
  \begin{tabular}{ c c c c c c c c c }
 \hline
%  \rowcolor[HTML]{f5e6ab}
 Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\
%  \rowcolor[HTML]{f5e6ab}
 Dataset & \multicolumn{2}{c}{CUB} &
 \multicolumn{2}{c}{NAB} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB}\\
 Split-mode & 
%  \rowcolor[HTML]{fcf9e8}
 Easy & Hard & Easy & Hard & Easy & Hard & Easy & Hard \\
 \hline
 GAZSL \cite{Yizhe_ZSL_2018} & \iffalse –lr 0.0001 –isval \fi 42.40 & \iffalse –lr 0.00005 –isval \fi 18.83& \iffalse –lr 0.0001 –isval) \fi 41.0 & \iffalse –lr 0.0001 –isval) \fi \textbf{9.34} & 39.13 & \textbf{15.16} & 28.71 & 6.43 \\
 CIZSL \cite{Mohamed_Creative_2019} & \iffalse (–lr 0.00005 –isval) \fi 41.38 & \iffalse  (–lr 0.0001 –isval)  \fi \textbf{18.99} & \iffalse –lr 0.0001 –isval) \fi 40.56& \iffalse (–lr 0.00005 –isval) \fi 9.29 & 38.65 & 14.93 & 27.86 & 6.69 \\
 \hline
 DGRZSL & \iffalse (–lr 0.0001 –isval \fi \textbf{42.44}& \iffalse  \fi 17.36 & \iffalse (–lr 0.0001 –isval) \fi \textbf{42.71} & \iffalse –lr 0.0001 –isval)  \fi 8.76 & \textbf{39.77} & 11.70 & \textbf{29.81} & \textbf{6.87} \\
 \hline
\end{tabular}
\caption{Zero-Shot classification results on CUB and NAB datasets}
  \label{tab:textual_results}
\end{table*}

==> figs/tab_textual_results_original_method.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}{ c c c c c c c c c }
 \hline
 Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\
 
 Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB}\\
 Split-mode & Easy & Hard & Easy & Hard & Easy & Hard & Easy & Hard \\
 \hline
 GAZSL \cite{Yizhe_ZSL_2018} & \iffalse (–lr 0.0001 ) \fi 44.08& \iffalse (–lr 0.0001 ) \fi 14.46 & \iffalse (–lr 0.0001 )  \fi 36.36 & \iffalse (–lr 0.0001 ) \fi 8.74 & 39.69 & \textbf{12.49} & 24.68 & 6.48 \\
 CIZSL \cite{Mohamed_Creative_2019} & \iffalse (–lr 0.0001 ) \fi 44.42& \iffalse (–lr 0.0001 ) \fi \textbf{14.8} & \iffalse (–lr 0.0001 ) \fi 36.85 & \iffalse (–lr 0.00005) \fi \textbf{9.04} & 39.46 & 11.85 & 24.83 & 6.48 \\
 \hline
 DGRZSL & \iffalse –lr 0.00005 ) \fi \textbf{45.48} & \iffalse –lr 0.00005 ) \fi 14.29 & \iffalse (–lr 0.0001 ) \fi \textbf{37.62} & \iffalse (–lr 0.0001 ) \fi 8.913 & \textbf{40.20} & 12.29 & \textbf{26.09} & \textbf{6.58} \\
 \hline
\end{tabular}
  \caption{\added{Zero-Shot classification results on CUB and NAB datasets using the original evaluation method}}
  \label{tab:textual_results_original_method}
\end{table*}
